Multi-scale reconstruction of undersampled spectral-spatial OCT data for coronary imaging using deep learning

Coronary artery disease (CAD) is a cardiovascular condition with high morbidity and mortality. Intravascular optical coherence tomography (IVOCT) has been considered as an optimal imagining system for the diagnosis and treatment of CAD. Constrained by Nyquist theorem, dense sampling in IVOCT attains high resolving power to delineate cellular structures/ features. There is a trade-off between high spatial resolution and fast scanning rate for coronary imaging. In this paper, we propose a viable spectral-spatial acquisition method that down-scales the sampling process in both spectral and spatial domain while maintaining high quality in image reconstruction. The down-scaling schedule boosts data acquisition speed without any hardware modifications. Additionally, we propose a unified multi-scale reconstruction framework, namely Multiscale- Spectral-Spatial-Magnification Network (MSSMN), to resolve highly down-scaled (compressed) OCT images with flexible magnification factors. We incorporate the proposed methods into Spectral Domain OCT (SD-OCT) imaging of human coronary samples with clinical features such as stent and calcified lesions. Our experimental results demonstrate that spectral-spatial downscaled data can be better reconstructed than data that is downscaled solely in either spectral or spatial domain. Moreover, we observe better reconstruction performance using MSSMN than using existing reconstruction methods. Our acquisition method and multi-scale reconstruction framework, in combination, may allow faster SD-OCT inspection with high resolution during coronary intervention.

==> chapters/abstract.tex <==
\begin{abstract}
Optical coherence tomography (OCT) is a biomedical imaging modality with technical merits such as high resolution, depth sectioning, and high speed acquisition. The endless effort to improve OCT systems has been made in increasing resolution and boosting acquisition speed. For intravascular coronary imaging, high resolution is required to visualize the critical features; high acquisition speed is required to reduce motion effects and the level of pain that a patient experiences. Swept source OCT (SS-OCT) systems offer a high imaging speed but reduced resolution; spectral domain OCT (SD-OCT) systems achieve higher resolution but lower imaging speed. In this paper, we propose an efficient spectral-spatial acquisition method and a multi-scale reconstruction framework, Multiscale-Spectral-Spatial-Magnification Network (MSSMN), which work together, boost the imagining speed for spectral domain OCT (SD-OCT) systems while maintaining their resolving power and reducing data storage consumption. Extensive experiments show that our framework is capable of recovering high quality OCT images from compressed images using multiple magnification factors in both spectral spatial domains. Moreover, our multi-scale reconstruction framework can process reduced OCT images using untrained magnification factors. With extensive experiments in human coronary OCT images, we demonstrated high accuracy, data efficiency, and magnification flexibility. Our work holds promise for improving OCT systems and facilitating clinical intervention. 
\end{abstract}

==> chapters/abstractV0.tex <==
\begin{abstract}
Coronary artery disease (CAD) is a type of cardiovascular disease which causes a high rate of human fatality. Intravascular optical coherence tomography (IVOCT) systems has been considered as an optimal imagining system for human coronaries, providing depth-resolved information to aid the diagnosis and treatment of CAD. %High scanning speed IVOCT systems are achieved via swept source optical coherence tomography (SS-OCT) but at a low resolution. Spectral domain optical coherence tomography (SD-OCT) has demonstrated its capability of resolving critical structures with a high resolution. 
However, the resolving power of IVOCT on critical sub-cellular structure is bottle-necked by the fact that there is no technology available to simultaneously maintain high spatial resolution and a fast scanning rate for coronary imaging.
%the image acquisition speed of SD-OCT needs to be improved for clinical coronary intervention. 
In this paper, we propose a viable spectral-spatial acquisition method to boost scanning speed of spectral-domain optical coherence tomography (SD-OCT), one OCT modality which has a high spatial resolution at sub-cellular level but conventionally not fast enough for IVOCT. Our acquisition method can be integrated to exiting SD-OCT systems without any hardware modifications. Additionally, we put forward a multi-scale reconstruction framework for resolving highly-compressed  ($\sim$6.25\%) OCT images with flexible magnification factors. We applied our acquisition method and reconstruction framework to human coronary samples with clinical features such stent and calcified lesions. With extensive experiments on coronary samples, we believe our acquisition method and multi-scale reconstruction framework are promising for improving SD-OCT systems in coronary intervention.
\end{abstract}

==> chapters/dummy.tex <==
\begin{table}
\centering
\caption{Results of Reconstructed OCT Image in Figure IV. The LR OCT Image is acquired with a factor of (4,4).}
\begin{tabular}{llllllllllllll}
 &  &                         &                                                    &                                                                                                                                   &                                                                                                                                   &                                                                                                              &  &  &  &  &  &  &   \\ 
\cline{3-7}
 &  & \diagbox{Method}{$(\hat{l},\hat{m})$} & Metrics                                            & (2,2)                                                                                                                             & (3,2)                                                                                                                             & (4,2)                                                                                                        &  &  &  &  &  &  &   \\ 
\cline{3-7}
 &  & Downsampled             & \begin{tabular}[c]{@{}l@{}}PSNR\\SSIM\end{tabular} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textcolor{blue}{\uline{21.9992}}\\\textcolor{blue}{\uline{0.2498 }}\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\uline{\textcolor{blue}{22.6984}}\\\uline{\textcolor{blue}{0.2745 }}\end{tabular}} & \begin{tabular}[c]{@{}l@{}}\textcolor{blue}{\uline{23.0206}}\\\textcolor{blue}{\uline{0.2844 }}\end{tabular} &  &  &  &  &  &  &   \\
 &  & MSSMN                   & \begin{tabular}[c]{@{}l@{}}PSNR\\SSIM\end{tabular} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textcolor{red}{22.9985}\\\textcolor{red}{0.3510 }\end{tabular}}                   & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textcolor{red}{23.4942}\\\textcolor{red}{0.3470 }\end{tabular}}                   & \begin{tabular}[c]{@{}l@{}}\textcolor{red}{23.5527}\\\textcolor{red}{0.3254 }\end{tabular}                   &  &  &  &  &  &  &   \\ 
\cline{3-7}
 &  &                         &                                                    &                                                                                                                                   &                                                                                                                                   &                                                                                                              &  &  &  &  &  &  &   \\
 &  &                         &                                                    &                                                                                                                                   &                                                                                                                                   &                                                                                                              &  &  &  &  &  &  &   \\
 &  &                         &                                                    &                                                                                                                                   &                                                                                                                                   &                                                                                                              &  &  &  &  &  &  &   \\
 &  &                         &                                                    &                                                                                                                                   &                                                                                                                                   &                                                                                                              &  &  &  &  &  &  &   \\
 &  &                         &                                                    &                                                                                                                                   &                                                                                                                                   &                                                                                                              &  &  &  &  &  &  &   \\
 &  &                         &                                                    &                                                                                                                                   &                                                                                                                                   &                                                                                                              &  &  &  &  &  &  &  
\end{tabular}
\end{table}








\begin{table}
\centering
\caption{Results of Acquiring OCT Images Using Different Strategies: Truncating the Spectrum from Centre and Dropping Spectral Data Uniformly.}
\label{table:tabMjNeo1}
\begin{tabular}{llllllll}
 &  &                             &                                                    &                                                                                                                                  &                                                                                                                                  &                                                                                                             &   \\ 
\cline{3-7}
 &  & \diagbox{Method}{$l$}         & Metrics                                            & \multicolumn{1}{c}{2}                                                                                                            & \multicolumn{1}{c}{3}                                                                                                            & \multicolumn{1}{c}{4}                                                                                       &   \\ 
\cline{3-7}
 &  & \multicolumn{1}{c}{Centre}  & \begin{tabular}[c]{@{}l@{}}PSNR\\SSIM\end{tabular} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textcolor{blue}{\uline{23.5410}}\\\textcolor{red}{0.5941}\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textcolor{red}{21.9768}\\\textcolor{red}{0.4517}\end{tabular}}                   & \begin{tabular}[c]{@{}l@{}}\textcolor{red}{21.2028}\\\textcolor{red}{0.3746}\end{tabular}                   &   \\
 &  & \multicolumn{1}{c}{Uniform} & \begin{tabular}[c]{@{}l@{}}PSNR\\SSIM\end{tabular} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textcolor{red}{24.0046}\\\textcolor{blue}{\uline{0.5871}}\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textcolor{blue}{\uline{19.0715}}\\\textcolor{blue}{\uline{0.3863}}\end{tabular}} & \begin{tabular}[c]{@{}l@{}}\textcolor{blue}{\uline{17.2993}}\\\textcolor{blue}{\uline{0.2922}}\end{tabular} &   \\ 
\cline{3-7}
 &  &                             &                                                    &                                                                                                                         &                                                                                                                                  &                                                                                                             &   \\
 &  &                             &                                                    &                                                                                                                         &                                                                                                                                  &                                                                                                             &   \\
 &  &                             &                                                    &                                                                                                                         &                                                                                                                                  &                                                                                                             &   \\
 &  &                             &                                                    &                                                                                                                         &                                                                                                                                  &                                                                                                             &  
  
\end{tabular}
\end{table}

\begin{table}
\centering
\caption{Results of Acquiring OCT Images Using Different Strategies: Truncating the Spectrum from Centre and Dropping Spectral Data Uniformly.}
\label{table:tabMjNeo1}
\begin{tabular}{llllllll}
 &  &                             &                                                    &                                                                                                                                  &                                                                                                                                  &                                                                                                             &   \\ 
\cline{3-7}
 &  & \diagbox{Method}{$l$}         & Metrics                                            & \multicolumn{1}{c}{2}                                                                                                            & \multicolumn{1}{c}{3}                                                                                                            & \multicolumn{1}{c}{4}                                                                                       &   \\ 
\cline{3-7}
 &  & \multicolumn{1}{c}{Centre}  & \begin{tabular}[c]{@{}l@{}}PSNR\\SSIM\end{tabular} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}23.5410\\0.5941\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}21.9768\\0.4517\end{tabular}} & \begin{tabular}[c]{@{}l@{}}21.2028\\0.3746\end{tabular} &   \\
 &  & \multicolumn{1}{c}{Uniform} & \begin{tabular}[c]{@{}l@{}}PSNR\\SSIM\end{tabular} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}24.0046\\0.5871\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}19.0715\\0.3863\end{tabular}} & \begin{tabular}[c]{@{}l@{}}17.2993\\0.2922\end{tabular} &   \\ 
\cline{3-7}
 &  &                             &                                                    &                                                                              &                                                                              &                                                         &   \\
 &  &                             &                                                    &                                                                              &                                                                              &                                                         &   \\
 &  &                             &                                                    &                                                                              &                                                                              &                                                         &   \\
 &  &                             &                                                    &                                                                              &                                                                              &                                                         &  
\end{tabular}
\end{table}

==> chapters/experimentsetup.tex <==
\section{EXPERIMENTAL SETUP AND EVALUATION METRICS}

==> chapters/introduction.tex <==
\section{INTRODUCTION}
Optical coherence tomography (OCT) is a high-resolution, depth-sectioning, and high-speed imaging modality that has been used in various research, such as biological, medical, and materials studies \cite{Boppart.2003}. Especially in cardiology, a consensus has been reached that OCT is capable of resolving superficial structures of vessel wall, hence providing useful information for the diagnosis and treatment of patients with coronary artery diseases \cite{Tearney.2012}. To facilitate OCT application, there are two directions to improve the performance of OCT imaging: spatial resolution and data acquisition. 

Better resolution for coronary imaging is generally desired. Current spatial resolution of intravascular OCT (10-20 $\mu$m) is restricted to cellular level, limiting the visualization of critical features and crucial clinical assessments of whether or not drug-eluting stents are covered with fibrin or endothelial cells. Patients with incomplete endothelial coverage are at increased risk of stent thrombosis. Current imaging technology lacks the power to perform assessment of such coverage. Differentiating endothelial cells from fibrin requires an imaging platform that can assess endothelial cell layer thickness $\sim$2 $\mu$m)\cite{finn2007pathological}. Because loss of endothelial lining is the pathological hallmark of plaque erosion, this limitation also precludes the adoption of endothelial cell absence as an OCT criterion for identification of plaque erosion.

Towards better resolution, there are continuous efforts to improve OCT systems by upgrading hardware or software. For example, recent development in light sources lead to increased optical resolution \cite{WuYuan.2016,Yuan.2017,Chong.2018} by broadening the bandwidth. Therefore, the improvement of resolution is bottlenecked by the current capability to produce a wide band light source. Besides, there is a tradeoff between spatial resolution and penetration depth. Improving spatial resolution from wider bandwidth will lead to a decreased penetration depth \cite{Chong.2018}. Moreover, hardware upgrading for an manufactured OCT system can be expensive and unpractical. In addition to hardware upgrades, there are software-based method to improve image quality to fine scale of resolution. Many digital signal processing or image processing algorithms, such as sparse representation\cite{J.Yang.2010,Fang.2013, Fang.2017,Abbasi.2018,Liu.2021}, have been proposed to reconstruct super-resolved OCT images. Recently, deep learning (DL) has risen in OCT image reconstruction/super-resolution tasks\cite{ChaoDong.2016,Lim.2017,WeiShengLai.2017,Zhang2018ResidualDN,Li.2018c,YulunZhang.2018b}. Deep learning models are specialized in fitting nonlinear mappings between the inputs and target outputs, which naturally suits the nonlinear reconstruction process. The success and potential of DL in reconstruction tasks has inspired medical imaging community; hence many researchers adopt DL based methods for improving qualities of OCT images\cite{Xu.2018,YongqiangHuang.2019,Zhou.2020,Z.Yuan.2020,S.Cao.2020,KaichengLiang.2020,Das.2020,Hao.2020b,HongmingPan.2020b,Jiang.2020,Qiu2020N2NSROCTSD}. However, simply pushing the resolution to its limit is not efficient enough for scanning and may cause additional computational/storage resources on regions that does not require resolution enhancement.

For an efficient scanning system, it is desired to maintain a flexibility to achieve resolutions at multiple arbitrary level. This requires different scale factors for studying different regions. One typical example is shown in Fig. \ref{fig:multi}, which is an OCT-histology match in a region of fibrous cap in human coronary. Here, we are interested in two regions: endothelial layer (gold box in a and green box in b) and lipid pool (white box in a and blue box in b). The two regions are magnified by different scales. As gatekeepers for passage of lipoprotein and leukocytes into intima, the endothelial layer needs to be magnified with a larger scale for accurate thickness determination. For lipid pools, however, thickness assessment is of less importance thus a lower magnification suffices. In fact, as a key factor to determine plaque vulnerability, the distance between pool edge to lumen is of interest. A distance of 65 $µ$m is widely used by pathologists as a cutoff minimal cap thickness for thin-cap fibroatheroma, a vulnerable plaque with high risk of rupture. Therefore, the lipid region needs a smaller scale magnification for shape determination (dash region)  within a larger field of view. 

Having a flexibility to magnify the image quality to multiple scale factors is critical for tissue characterization. With previous DL methods, a new networks has to be individually trade if there is a need for a new scale factor. %required to achieve varying magnification factors. 
Thus, multiple DL networks need to trained if analysis with multiple scale factors is required. Noticably, training multiple DL models is computationally expensive. Besides, previous DL method can not process magnification factors which are not included in the training set. Thus, it is in unmet need to develop a single neural work for multi-scale image reconstruction/magnification.
%(YG: multi-network is not the best solution, we need single network) refer to the meta-sr paper. Untrained factors
\begin{figure*}[t]
\centering
\includegraphics[width=17 cm]{figures/multi.eps}
\caption{Representative of a pairwise match between coronary OCT image (left) and its histology (right). Two regions are magnified with different scales for coronary analysis. Two regions need to magnified at two specifice levels for tissue characterization. scale bar: 200 $\mu$m.}
\label{fig:multi}
\end{figure*}


Towards data acquisition, it is also important to sample less data while maintaining image quality of reconstruction. This will boost data acquisition speed, decrease workload for data storage/transmission, and reduce motion effect. In previous research, OCT data compression were carried out from two separate perspectives: spectral domain compression \cite{DBLP:journals/corr/SimonyanZ14a, Fang.2013,Fang.2017, PengfeiGuo.2020, Ronneberger.2015} and spatial domain compression \cite{ AntoniaLichtenegger.2021,Zhang.2021b}. Spectral domain downsampling was proposed but limited to comparatively small factors. Spatial domain downsampling works on the full-size image and thus requires storage and computational resource for the whole spectrum. However, how to jointly reduce data from spectral domain and spatial domain remains elusive. 

In this paper, we put forward an efficient spectral-spatial domain acquisition method for Spectral Domain-OCT (SD-OCT) systems. Our method is effectively reduce the data size in both spectral domain and spatial during data acquisition. %when a OCT system captures spectrum data during scanning, we truncate the spectrum data by a given spectral acquisition factor $i$ and then we skip A-lines by a spatial acquisition factor of $j$. By skipping A-lines, the data acquisition speed is improved; by truncating spectrum, data storage consumption is reduced. 
Our method can be easily integrated into any data acquisition workflow of SD-OCT systems without introducing extra computational overhead. Additionally, We propose a single neural network, namely Multiscale-Spectral-Spatial-Magnification Network (MSSMN), with the flexibility to improve OCT images to multiple arbitrary scale factors. Inspired by super-resolution technology, MSSMN magnifies compressed information in both spectral and spatial domains with any arbitrary magnification (reconstruction) factors. %$(\hat{i},\hat{j})$. 

Our contributions are as follows:
\begin{itemize} 
\item We propose a novel method to efficientize OCT data acquisition, collaboratively reduce data in spectral domain and spatial domain. The proposed method improves acquisition speed while reducing data storage consumption. Our method is fully integrated to the workflow of SD-OCT systems and introduce no extra computational overhead.
\item We devise a unified network, MSSMN, to address the issue of simultaneously reconstructing compressed OCT images in both spectral and spatial domains. To the best of our knowledge, it is the first multi-scale OCT reconstruction framework in spectral-spatial domain, providing flexibility to process compressed OCT images for multiple magnification factors.
\item The proposed multi-scale reconstruction framework achieves better performance compared to previous method functioning on single magnification factor. Our framework functions on arbitrary magnification factors, even those factors that are not included in training dataset.
\item We proposed the first super-resolution neural network for coronary OCT imaging with an aim to highlight pathological pattern such as calcified region, stent structure, and lipid region. %We conducted extensive experiments on human coronary OCT and demonstrate the spectral-spatial acquisition method is much more efficient in reconstruction performance than solely reduce data in spatial or spectral domain. 
\end{itemize}
